BBS: A Blockchain Big-Data Sharing System

Chain of custody is needed to document the sequence of custody of sensitive big data. In this paper, we design a blockchain big-data sharing system (BBS) based on Hyperledger Fabric. We denote the data stored outside of a ledger for sharing as "off-state" and "big data" (referring to extremely large data) is in this category. In our off-state sharing protocol, a sender registers a file with BBS for sharing. To acquire the file, an authenticated and authorized receiver has to use transactions and interacts with BBS in four phases, including the file transfer request, encrypted file transfer, key retrieval, and file decryption. The corresponding transactions are recorded in the ledger and serve as chain of custody to document the trail of the data. Compared with related work, BBS can perform the four phases autonomously. It utilizes the permissioned blockchain, i.e. Hyperledger Fabric, for access control and can defeat dishonest receivers. We design and implement a prototype of BBS for big file sharing. Extensive experiments were performed to validate its feasibility and performance.

==> sections/trash/sec2_relatedwork.tex <==
\section{Related Work}
\label{sec::related_work}

In this section, we investigate the existing blockchain-based data sharing systems and their drawbacks. 

% Most related work on blockchain-based data sharing systems does not focus on the big file sharing. It does not address the specific challenges in big file sharing or solve the problem.

We group existing blockchain-based data sharing schemes into two categories: on-chain schemes and off-chain schemes. On-chain data sharing schemes store shared data in ledgers and are not suitable for big file sharing due to ledger storage limitations. Off-chain data sharing schemes store shared data outside the blockchain system and the blockchain system only manage the data access token. Off-chain schemes have no storage limitation but these off-chain schemes either fail to design a secure data access protocol or put additional computational work on senders and receivers and involve in multiple interactions to share one file.

% \subsection{Data Sharing in Ledgers}
\subsection{Data Sharing On-Chain}
In on-chain data sharing schemes, shared data is stored in the world state. The smart contracts in the blockchain system maintain the data in the world state and control the data access. Users set or get shared data through proposing transactions to interact with the blockchain system. Transactions are the carriers of the shared data. 
Wang et al.\cite{wang2020blockchain} utilize the blockchain system as the back end to transmit and store data from the front-end wireless body area networks (WBAN). All blockchain nodes maintain the same data and all participants such as doctors and insurance providers share the same WBAN data.
Zhang et al. \cite{zhang2018towards} propose a blockchain-based secure and privacy-preserving personal health information (PHI) sharing scheme. The original PHI records are stored in the ledger of the private blockchain of each hospital, and the consortium blockchain keeps records of the indexes of the PHI. 
Jiang et al. \cite{jiang2018blochie} propose a blockchain-based platform for healthcare information exchange. They use two loosely coupled blockchains to handle different kinds of healthcare data, including highly sensitive electronic medical records (EMRs) and personal healthcare data (PHD). 
All these existing schemes store shared data in the world state, and are not suitable for big file sharing applications because big files cannot be stored in blockchain ledgers due to the storage limitation as analyzed in Section \ref{sec::Storage_Limitations}.


% \subsection{Data Sharing Outside Ledgers}
\subsection{Data Sharing Off-Chain}
There are systems that store shared data outside the blockchain systems. The blockchain system only manage the data access tokens and users access the shared data off-chain utilizing access tokens. 

\subsubsection{Token-based Scheme}
In some token-based off-chain data sharing schemes, a user proposes a transaction to request a data access token and the blockchain system returns an access token to the user. The user then uses the access token to request the shared data from a data center, which is outside of the blockchain system. 
% Xia et al. \cite{xia2017medshare} propose a blockchain-based solution to sharing medical data among cloud service providers. In their design, smart contracts retrieve requested data from existing database infrastructure, outside of a blockchain system. The retrieved results are recorded in the blockchain. It is impractical to record big files in a blockchain. 
Lu et al. \cite{lu2019blockchain} design a blockchain empowered privacy-preserved data sharing architecture for industrial IoT. 
% They exploit the privacy-preserved federated learning algorithm to learn the data model and share the data model instead of revealing the actual data. 
They use the blockchain to retrieve and manage the accessibility of data.
Zhang et al. \cite{zhang2018fhirchain} choose to store and exchange only reference pointers of the sensitive data in the blockchain. A data requester should first get a token from the blockchain system and then use the token to access original data in the database outside the blockchain. 

% \textit{Drawbacks of Token-based Scheme:}
Such token based file sharing blockchain model does not have storage limitations, and may be used for big file sharing. But such model requires a centralized and trusted data provider. The data center is controlled by the data provider.
The Blockchain system has no control over the actual data access and cannot know the status of data sharing, e.g. whether the data is actually shared. The integrity of chain of custody cannot be ensured and audited.
% (ii) There is no detailed presentation of the actual protocol in \cite{zhang2018fhirchain}.
% (iii) The data center based approach is not flexible. In scenarios such as file sharing in biomedical fields, data owners may want to share data between their workstations. 
They also fail to consider security requirements such as dealing with dishonest users, and fail to design a protocol for secure data sharing.

\subsubsection{Fair Exchange Protocol for Selling Large Files}
FairSwap \cite{dziembowski2018fairswap} is a protocol for fair exchange of digital goods in a public blockchian which involves build-in cryptocurrencies, i.e. Ethereum. It can be applied for fairly selling large files. A receiver has to pay a sender for a received correct file. In Ethereum, users need pay fees for executing the smart contract. More complex the smart contract is and more larger the processed data is, more cryptocurrencies users need pay. To reduce the cryptocurrencies cost, FairSwap outsources heavy computation work off-chain to senders and receivers, such as file transfer and encryption/decryption computation. The blockchain system only conducts light-weight computations such as cryptocurrencies transfer and encryption keys exchange. Normally, off-chain behaviors are trustless. To avoid a receiver pays for a wrong file, a concise proof of misbehavior is designed for a sender to complain to the smart contract in a limited period of time, and the smart contract judges the cases and refunds the locked cryptocurrencies. To produce concise proof of misbehavior, FairSwap involves in some additional complex computational work, such as circuits encoding, Merkle tree proof construction, file splitting and so on.
% A sender off-chain transfers an encrypted file to a receiver. The receiver evaluate the encrypted file hash and locks some cryptocurrencies. Then the sender reveals the encryption keys to the blockchain system. The receiver can instantly get these keys in the public blockchain, and in the same time the smart contract transfers some previously locked cryptocurrencies to the sender. 
% FairSwap \cite{dziembowski2018fairswap} and Optiswap \cite{eckey2020optiswap}

% \textit{Drawbacks of Fair Exchange Protocol:}
FairSwap is designed for digital goods, such as large files, exchange on a public blockchain system which has build-in cryptocurrencies. We summarize the main drawbacks of FairSwap as follows:
\begin{enumerate}
\item FairSwap requires a secure channel to transfer digital goods. In a public blockchain system, all data is public. When the encryption keys are revealed to the smart contract by the sender, everyone including the receiver can get the encryption keys used for file decryption. Once the encrypted file is revealed to others during off-chain transfer process, the original file will be revealed. Therefore, a secure channel is required.
\item In FairSwap, digital goods exchange cannot be conducted automatically without off-chain interactions between involved parties. Digital goods are transferred off-chain, where involved parties conduct multiple interactions with each other beyond interactions with the blockchain system. This requires the involved parties previously know each other well and negotiate well with each other. Therefore, such digital goods exchange cannot be conducted automatically without off-chain interactions between involved parties. 
\item In the blockchain system which has build-in cryptocurrencies, executing smart contracts is usually costly. To reduce such costs, FairSwap overall involves additional computational works to generate a concise proof of misbehavior. 
\item In the public blockchain system, i.e. Ethereum, users are usually anonymous. The public/private key is only related with a pseudonym. There is no access control mechanism based on user identities. FairSwap only sells a file whose hash matches with a fixed value. There is no more access control rules based on user identities. 
\item FairSwap does not consider the case where a sender provides a wrong key to the contract. In this case, a receiver cannot decrypt received data to generate a proof of misbehavior.
\end{enumerate}

secure design is not approporiate for our application

autonomous

system seperat

segregate





In our scenario, a consortium of organizations cooperate together to sharing some sensitive big data. They desire to use the blockchain to record the chain of custody of shared data. They do not trade the data for money with each other. We design an off-state sharing system for large file sharing based on a permissioned blockchain system which does not involves cryptocurrencies. In our system PBOSS, only the involved sender and receiver can get the encryption keys. PBOSS does not require a secure channel to transfer files; In the permissioned blockchain system, there is no build-in cryptocurrencies and executing smart contract is free. We delegate the smart contract to do all necessary computations and no additional computational work is outsourced to senders and receivers. The file can be automatically shared without a receiver interacting with a sender during the sharing process; In a permissioned blockchain system, users are non-anonymous, and there are many build-in access control mechanisms. Based on the user identity, we can utilize the smart contract to define more rules over large files access control. Wang et al. \cite{PDCFabric} find misuse of PDC in Fabric may endanger a blockchain system and PBOSS avoids such issues in the implementation.



% These existing schemes do not focus on big file sharing. They also fail to consider security requirements such as dealing with dishonest users, and fail to design a protocol for secure off-state sharing.
% Wang et al. \cite{PDCFabric} find misuse of PDC in Fabric may endanger a blockchain system and BOSS avoids such issues in the implementation.

% design a specific protocol to guarantee the safety of large files transfer between trustless parties considering dishonest participants.









==> sections/trash/sec4.tex <==
\delete{
\subsubsection{Scenario 1: A receiver denies that it has received a transferred file}

In our four-phase file sharing protocol, the receiver has to obtain $K_{aes}$ in order to decrypt the encrypted file $F_{enc}$, which the sender sends.
%the receiver should get the access permission of $K_{aes}$ and then query $K_{aes}$ to decrypt $F_{enc}$ to get $F$.
$K_{aes}$ is stored in the world state of the ledger, which guarantees its integrity because of the underlying blockchain framework. That is, once a receiver proposes ``Tx: key access", the receiver will definitely receive $K_{aes}$. The user can then propose ``Tx: file decryption" to get $F$. In this scenario, the auditor can find out the fact by retrieving ``Tx: key access" in the blockchain. If the receiver receives $F_{enc}$ but does not propose a transaction to request $K_{aes}$, the receiver can not get the original file $F$. In this situation, we regard it as the receiver does not receive the file $F$. 


\subsubsection{Scenario 1: Dishonest Sender}
As discussed in \textit{Challenge 3---Security Requirement}, the sender may wrongly declare that she/he has transferred the file but actually not.
%We define the policy to identify if the sender has transferred the file as follows.

%Once the \texttt{Encryption Key} entry is recorded in the world state, it means the sender claims that she/he has transferred the file.
%\textit{Security Analysis:} 
In our four-phase file sharing protocol, an \texttt{Encryption Key} entry will be recorded in the world state while the sender transfers the encrypted file to the receiver. The world state is always updated through transactions. The corresponding transaction ``Tx: transfer file" is recorded in an immutable blockchain. 
%Auditors can find out the fact by retrieving the corresponding transaction in the blockchain. 
If the sender only sets the \texttt{Encryption Key} entry but does not send the encrypted file, the receiver will not request the encryption key since she/he does not receive any encrypted file. The file sharing process will not be completed.
It can not benefit the sender. Therefore, the sender has no incentive to only set the encryption key to claim he has sent the file but not actually sends $F_{enc}$. 


\subsubsection{Scenario 3: Wrong Files}
In \textit{Challenge 3---Security Requirement}, a receiver may transfer a wrong file. The receiver may claim that the received file is not the desired one. We define the policy to identify if the transferred file is consistent with \texttt{File Profile} in world state as follows:

% The receiver may claim that the received file is not the desired one. We define the policy to identify if the transferred file is consistent with the file profile in the world state as following: 

\textbf{Policy 3. File Correctness:} The receiver provides the received encrypted file $F_{enc}$ and \texttt{Encryption Key} in world state to an auditor. Auditor can check if the \texttt{Encryption Key} match the PDC hash in the auditor node's world state who is a PDC non-member. If the \texttt{Encryption Key} is the correct one, an auditor can judge the file correctness according to the following three conditions: 
\begin{enumerate}
 
\item[i)] $F_{enc}$ can pass the signature verification as show in formula (\ref{eqn::verify_rsa}). That is the $R$ is $True$.
\begin{eqnarray}
R = Verify(Signature(F_{enc}), H(F_{enc}), K_{public})
\label{eqn::verify_rsa}
\end{eqnarray}

\item[ii)] $F_{enc}$ match the $H(F_{enc})$ in \texttt{Encryption Key};

\item[iii)] The plaintext $F$ decrypted from $F_{enc}$ matches $H(F)$ in \texttt{File Profile} recorded in world state. 
\end{enumerate}
If any one condition is violated, the transferred file is incorrect. If all conditions are satisfied, the transferred file is correct.

\textit{Security Analysis:} 
The information used to audit includes $F_{enc}$ and some data in world state. $F_{enc}$ is in off-state but can be verified through $H(F_{enc})$ in world state. Data in world state is safe and verifiable. 
An auditor can identify who perform dishonestly so as to ascribe blame.
If condition i) is violated, it means the receiver provides wrong information to the auditor. 
If condition i) is satisfied but condition ii) is violated, it means that the sender sends wrong $F_{enc}$ that does not match $H(F_{enc})$ in the world state.
If condition iii) is violated and condition i) and ii) are satisfied, it means the sender sends wrong file that does not match the file profile in the world state. 

In the case of that both participants behave honestly but the receiver is unsatisfied with the file content, the issue should be solved by authoritative arbitration institution and the blockchain system only provides proof.

% \subsection{Apply Traitor Tracing and Water Markers Techniques}

}

==> sections/trash/sec5_system.tex <==
\section{Proof-of-Concept Implementation Based on Hyperledger Fabric}
\label{sec::poc_system}

\Fu{Can we use Etherum and Bitcoin to implement this system? May need to merge this section into last section}
%This section presents details of the proof of concept (PoC) implementation of the system.
We design a prototypical big file sharing system based on Hyperledger Fabric.
%We first briefly present features of Hyperledger Fabric that fit our big files sharing mechanism. 
Then we introduce the PoC system framework, workflow and some implementation details.

% Hyperledger Fabric is a popular permissioned blockchain framework, which only authorized participants can involve in.

\subsection{System Framework and Workflow}
\label{sec::systemFramework}

Framework of the PoC system is shown in Fig. \ref{fig::framework}. Three organizations, i.e. org1, org2 and org3, cooperatively build this system. Org1 and org2 respectively represent the sender and the receiver, and each party contributes one peer node and one client node. Org3 represent an auditor organization, and contribute one peer node and one orderer node. Smart contract is also called chaincode in Fabric. We implement our off-state integration mechanism using chaincode, and adopt \textit{SFTP} \cite{sftp_Wikipedia} to conduct file transfer.

\subsubsection{Peer Modifications}
In our system, peer nodes are different from the traditional Hyperledger Fabric peer nodes. We integrate an off-state and the \textit{SFTP} service to some peer nodes. We create an off-state storage space in the chaincode's workspace. So the chaincode can interact with the local off-state and operate on it. Nodes in Hyperledger Fabric run in Docker containers\cite{anderson2015docker} without \textit{SFTP} service. We install \textit{SFTP} service \cite{sftp_Wikipedia} in some peer nodes. 
% In Hyperledger Fabric, chaincode is a program written by general-purpose programming languages, which usually have \textit{SFTP} service library. 
So file owners can upload files to off-state, and the chaincode can invoke \textit{SFTP} to transfer files in local off-state.

\subsubsection{Transaction Workflow}

%In Hyperledger Fabric, as shown in Fig.\ref{fig::framework}, a common transaction workflow is as follows: 1. A client proposes a transaction proposal to some peer nodes, i.e. endorsers, specified by the endorsement policy; 2. Endorsers execute the chaincode, sign the execution results, and return the results with corresponding signatures to the client as proposal responses; 3. If the returned execution results from different endorsers are the same, the client assembles a transaction and sends it to the orderer node. 4. The orderer node collects multiple transactions in the same time, bundles transactions into a new block, and distribute the new block to all peers including both endorsers and non-endorsers. 5. All peers validate the transactions in the received new block. If the transaction is valid, the peer will update world state according to execution results. After validating all transactions, each peer appends the new block to a blockchain. 

In our three-phase file sharing event, one event involves four transactions as shown in Fig. \ref{fig::Module2}. All involved transactions follow the same common transaction workflow. The only difference is that endorsers are different in Steps 1 and 2. according to different endorsement policy setting. 


\subsection{Endorsement Policy Setting}
\label{sec::Endorsement_Policy_Set}

We illustrate the endorsement policy setting for involved four transactions in one file sharing event, including ``Tx: request permission", ``Tx: transfer file", ``Tx: request key" and ``Tx: decrypt file". The default chaincode-level endorsement policy is set as AND(Org1MSP, Org2MSP), which means peer nodes from both org1 and org2 need endorse a transaction. Note that org3 does not involve in any endorsing and only synchronizes the ledger data, i.e. world state and blockchain. In the following illustration, we assume Peer1 is the sender and Peer2 is the receiver.

% \subsubsection{File Uploading Event}
% In Module 1, when add a new file to the off-state, the smart contract should record the File Profile entry to the world state. The corresponding entry is $\langle$file\_name, $H(F)$, owner, access\_rule, description$\rangle$. The smart contract should read the file from the off-state and calculate the file hash. Since peer nodes only maintains their own files, only the file's owner peer can get the hash information. So the key-level policy for this entry should be customized. For example, when the user add file 1 to the Peer 1, the key-level policy for file 1 profile entry should be AND(Org1MSP), which mean only Peer 1 acts as the endorser and execute the smart contract. Though other peer nodes do not execute the smart contract, they will also store the entry in the world state and store the corresponding transaction in the blockchain. 

% \subsubsection{Module 2 implementation}
% Transferring files involves three phases:

\subsubsection{Tx: request permission}
During this transaction, chaincode verifies if pre-defined access control rules are satisfied, and records the verification result in an \texttt{Event} entry. This should be conducted by both sender and receiver, i.e. Peer1 and Peer2. So the endorsement policy for this transaction uses the default chaincode-level endorsement policy, i.e. AND(Org1MSP, Org2MSP). 

\subsubsection{Tx: file transfer}
During this transaction, chaincode conducts encrypting file, transferring file and writing \texttt{Encryption Key} to world state. $K_{aes}$ in \texttt{Encryption Key} should be kept only by the sender and other peers only store the hash. So \texttt{Encryption Key} should be set as a PDC and only the sender node Peer1 is the PDC member. Besides, only Peer1 owns the file to be encrypted and transfered. So the endorsement policy for this transaction should be customized as a collection-level policy and the policy should be AND(Org1MSP). That's only Peer1 performs as an endorser.

\subsubsection{Tx: request key}
During this transaction, chaincode should reset the PDC member of \texttt{Encryption Key} and add the receiver Peer2 to the PDC member. Then the receiver will own the original $K_{aes}$. The sender Peer1 should act as the endorser since it is the only original member of \texttt{Encryption Key}. The endorsement policy for this transaction should be AND(Org1MSP).

\subsubsection{Tx: query key and decrypt}
During this transaction, chaincode queries \texttt{Encryption Key} in world state to decrypt the encrypted file in the off-state. It is the receiver Peer2 who needs to decrypt the received encrypted file. And Peer2 now owns $K_{aes}$. So the endorsement policy for this transaction should be set as AND(Org2MSP).

% \subsubsection{Stage 3 implementation}

% If some disputes occur, the auditer organization will involved. The audit organizaton does not involve in the file uploading and file transferring. It only records all entries in its world state and all transactions in its blockchain. The auditer peer only conducts audit. So the smart contract running in the Peer 3 is different from Peer 1 and Peer 2. This can be implemented due to the customizable smart contracts feature in Hyperledger Fabric. According to the three audit policies in Section \ref{sec::stage3}, the smart contract needs query the file profile entry, encryption key entry and the transaction history. All these information locates in the auditer peer node, so the endorsement policy can be set as AND(Org3MSP).

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{figures/fig_framwork.pdf}
\caption{Framework of big files sharing system based on Hyperledger Fabric
\Fu{Font too small. Shall be similar to body text font size}}
\label{fig::framework} 
\end{figure}

% \subsection{Big Files Sharing Workflow}

%The whole file transfer process involves multiple transactions. At stage 1, the client proposes a transaction to record the new file uploaded to the off-state. 
%At stage 2, the receiver's client first proposes a transaction to request the transfer agreement. Then the sender's client proposes a transaction to transfer the file from one node to the other node. Next the receiver's client proposes a transaction to request the encryption key and at last proposes another transaction to query the encryption key and decrypt the received file. 
%At stage 3, the client can propose a transaction to conduct one policy check according to different scenarios.



%All involved transactions in the whole file transfer process follow the same common transaction workflow in Hyperledger Fabric. The only difference is that the corresponding endorsement policy involved in different transactions are different since these transactions operate different entries in the world state. We have analysed the endorsement policy setting for different entries in the last Section \ref{sec::systemFramework}. The common transaction workflow is as following: i) The client proposes a transaction proposal to the endorsers defined by the endorsement policy; ii) Endorsers execute the smart contract, sign the execution results, and return the results with corresponding signatures to the client; iii) If the returned results from different endorsers are the same, the client assembles a transaction and sends it to the orderer node. iv) The orderer node collects multiple transactions in the same time, blindly bundles transactions into new blocks, and distribute the new block to all peers including both endorsers and non-endorsers. v) All peers validate the transactions in the received new block. If the transaction is valid, the peer will update the data in the world state and append the new block to the blockchain. 

==> sections/trash/sec7_discussion.tex <==
\section{Discussion}
\label{sec::discussion}

In this section, we discuss the impact of chaincode execution timeout on big file sharing, potential implementation of BOSS with other blockchain frameworks, difference between off-state and off-chain and out-of-band distribution of received files by users. \looseness=-1

\subsection{Chaincode Execution Timeout}

% Current blockchain frameworks are not specifically designed to manage large data and high-latency transactions. 
% We summarize the problems in evaluation experiments, which indicates future improvements for the blockchain framework used to build the large file sharing system.

In Fabric, chaincode has a system wide execution timeout setting. The default timeout value is $30s$. In BOSS, the chaincode invokes SFTP for file transfer and waits for SFTP to finish. 
However, $30s$ is far from enough for transferring a big file and the chaincode will time out.
This timeout setting can be changed in the docker configuration file of Fabric, but cannot be changed at runtime based on the size of the file.
We find setting the timeout to infinity does not work in Fabric either and plan to revise Fabric as future work so that we can change the timeout flexibly.

\subsection{Implementation based on Other Blockchain Frameworks}

Bitcoin is not appropriate to implement BOSS. First, Bitcoin is a permissionless blockchain system. It is hard to implement access control. Second, Bitcoin essentially is a blockchain-based cryptocurrency application. There is no existing mechanism like smart contracts for programming. It will be a challenge and tedious to develop other applications over it.

Enterprise Ethereum \cite{enterpriseEthereum} can be used to implement a blockchain off-state sharing system.
Enterprise Ethereum \cite{Hyperledger_Besu}\cite{goquorum} is a permissioned blockchain framework for enterprise applications. It has many similar features to Fabric.
First, there is a private world state as well as a public world state for each enterprise Ethereum node. The private world state is only shared within a private group.
Enterprise Ethereum provides a private transaction manager, which can be used to keep transactions private among a private group. 
The private world state is similar to PDC in Fabric and can be used to manage the encryption key access required by BOSS.
Second, there is a private contract mechanism. A private contract is only available and executed on a subset of nodes. This is actually similar to customizable chaincode in Fabric and is flexible for the sender/receiver peers to implement their own business logic.
Third, the language of smart contracts is Solidity \cite{solidity_Wikipedia} in Ethereum. Solidity is a Turing-complete program language which can be used to implement a business logic. 

% \subsection{Difference between Off-State and Off-Chain}

% Off-state is different from off-chain \cite{poon2016bitcoin,coleman2018counterfactual,dziembowski2018general}, and existing off-chain protocols can not be utilized to ensure the safety of off-state data. 
% The off-chain technique is designed to scale the blockchain systems and improve transaction throughput. 
% It constructs transactions off-chains, and submits one transaction containing the final results to update the world state.
% Essentially, the off-chain protocol is designed to guarantee the safety of the world state. 
% The well-known off-chain technique is the payment channel in Bitcoin \cite{poon2016bitcoin}. A payment channel first locks some on-chain cryptocurrencies, i.e. the UTXOs state. Then it constructs transaction off-chains to conduct micropayments using locked cryptocurrencies, but does not commit these transactions involving micropayments to the blockchain. At last, it commits one transaction that represents final micropayment results to the main blockchain to update the UTXOs world state.
% Off-chain can not solve the storage limitation issues or be used for big file sharing. 

\subsection{Out-of-band Data Distribution}

Once the file is transferred to a user through BOSS, the user may stealthily send the file to other parties through out-of-band commnunication but not through BOSS. It will be hard to trace those files. This is a generic problem in data sharing, not specific to our system. Potential solutions include digital watermark \cite{van1994digital} and traitor tracing \cite{boneh1999efficient}, which adds some additional information to the files. Another strategy will be to limit the user capabilities with the files to particular workstations and use physical security and particular configurations that allow file transfer only through BOSS.
%This is out of scope of this paper and we mainly focus on safety of file sharing process.



